Deep Learning and Machine Learning with GPGPU and CUDA: Unlocking the Power of Parallel Computing

General Purpose Graphics Processing Unit (GPGPU) computing plays a transformative role in deep learning and machine learning by leveraging the computational advantages of parallel processing. Through the power of Compute Unified Device Architecture (CUDA), GPUs enable the efficient execution of complex tasks via massive parallelism. This work explores CPU and GPU architectures, data flow in deep learning, and advanced GPU features, including streams, concurrency, and dynamic parallelism. The applications of GPGPU span scientific computing, machine learning acceleration, real-time rendering, and cryptocurrency mining. This study emphasizes the importance of selecting appropriate parallel architectures, such as GPUs, FPGAs, TPUs, and ASICs, tailored to specific computational tasks and optimizing algorithms for these platforms. Practical examples using popular frameworks such as PyTorch, TensorFlow, and XGBoost demonstrate how to maximize GPU efficiency for training and inference tasks. This resource serves as a comprehensive guide for both beginners and experienced practitioners, offering insights into GPU-based parallel computing and its critical role in advancing machine learning and artificial intelligence.

==> review_notes.tex <==
Ming Li: (all implemented)
1.1: Add NPU and FPGA, add plots and explanation

GPU Programming Models Beyond CUDA: After 5.4, before 5.5 Conclusion. The new section introduces OpenCL, Vulkan, and Metal as alternatives to CUDA, with code examples and comparisons.

High-Level GPU Libraries Overview: Add at the beginning of Chapter 7 as a prelude to specific GPGPU applications, focusing on libraries like cuBLAS, cuDNN, TensorRT, PyTorch, and TensorFlow.

GPU Virtualization and Cloud Computing: After 7.5, create a new section that explores how GPUs are used in cloud platforms and the importance of GPU virtualization for scalable workloads.

L3 Cache Allocation Strategies: Expand 3.4 by integrating L3 cache management strategies and their impact on CPU and GPGPU performance, emphasizing static vs. dynamic allocation and real-world use cases.


